Link Scheduling using Graph Neural Networks

Efficient scheduling of transmissions is a key problem in wireless networks. The main challenge stems from the fact that optimal link scheduling involves solving a maximum weighted independent set (MWIS) problem, which is known to be NP-hard. In practical schedulers, centralized and distributed greedy heuristics are commonly used to approximately solve the MWIS problem. However, most of these greedy heuristics ignore important topological information of the wireless network. To overcome this limitation, we propose fast heuristics based on graph convolutional networks (GCNs) that can be implemented in centralized and distributed manners. Our centralized heuristic is based on tree search guided by a GCN and 1-step rollout. In our distributed MWIS solver, a GCN generates topology-aware node embeddings that are combined with per-link utilities before invoking a distributed greedy solver. Moreover, a novel reinforcement learning scheme is developed to train the GCN in a non-differentiable pipeline. Test results on medium-sized wireless networks show that our centralized heuristic can reach a near-optimal solution quickly, and our distributed heuristic based on a shallow GCN can reduce by nearly half the suboptimality gap of the distributed greedy solver with minimal increase in complexity. The proposed schedulers also exhibit good generalizability across graph and weight distributions.

==> macros.tex <==

% circular convolution
\def\cast{{
   \mathord{
      \hbox to 0em{
         \ooalign{
	   \smash{\hbox{$\ast$}}\crcr
	   \smash{\hskip-1pt\Large\hbox{$\circ$}} }
	 \hidewidth}
      \phantom{\bigcirc}
} }}
% AMIR's macros


% Hatted english letters
\newcommand{\ghat}{\mbox{$\bm \hat g$}}

%abbreviations for greek letters
\newcommand{\bsigma}{{\bm\sigma}}


\newcommand{\ga}{\alpha}
\newcommand{\gb}{\beta}
\newcommand{\grg}{\gamma}
\newcommand{\gd}{\delta}
\newcommand{\gre}{\varepsilon}
\newcommand{\gep}{\epsilon}
\newcommand{\gz}{\zeta}
\newcommand{\gzh}{\mbox{$ \hat \zeta$}}
\newcommand{\gh}{\eta}
\newcommand{\gth}{\theta}
\newcommand{\gthh}{\mbox{$ \hat \theta$}}
\newcommand{\gi}{iota}
\newcommand{\gk}{\kappa}
\newcommand{\gl}{\lambda}
\newcommand{\glh}{\mbox{$ \hat\lambda$}}
\newcommand{\gm}{\mu}
\newcommand{\gn}{\nu}
\newcommand{\gx}{\xi}
\newcommand{\gp}{\pi}
\newcommand{\gph}{\phi}
\newcommand{\gr}{\rho}
\newcommand{\gs}{\sigma}
\newcommand{\gsh}{\hat \sigma}
\newcommand{\gt}{\tau}
\newcommand{\gu}{\upsilon}
\newcommand{\gf}{\varphi}
\newcommand{\gc}{\chi}
\newcommand{\go}{\omega}

%Uppercase Greek

\newcommand{\gG}{\Gamma}
\newcommand{\gD}{\Delta}
\newcommand{\gTh}{\Theta}
\newcommand{\gL}{\Lambda}
\newcommand{\gLh}{\mbox{$ \hat\Lambda$}}
\newcommand{\gX}{\Xi}
\newcommand{\gP}{\Pi}
\newcommand{\gS}{\Sigma}
\newcommand{\gU}{\Upsilon}
\newcommand{\gF}{\Phi}
\newcommand{\gO}{\Omega}

%Uppercase bold Greek

\def\bm#1{\mbox{\boldmath $#1$}}
\newcommand{\vga}{\mbox{$\bm \alpha$}}
\newcommand{\vgb}{\mbox{$\bm \beta$}}
\newcommand{\vgd}{\mbox{$\bm \delta$}}
\newcommand{\vgrg}{\mbox{$\bm \gamma$}}
\newcommand{\vge}{\mbox{$\bm \epsilon$}}
\newcommand{\vgl}{\mbox{$\bm \lambda$}}
\newcommand{\vgr}{\mbox{$\bm \rho$}}
\newcommand{\vgrh}{\mbox{$\bm \hat \rho$}}
\newcommand{\vgrt}{\mbox{$\bm {\tilde \rho}$}}

\newcommand{\vgt}{\mbox{$\bm \gt$}}
\newcommand{\vgth}{\mbox{$\bm {\hat \tau}$}}
\newcommand{\vgtt}{\mbox{$\bm {\tilde \tau}$}}
\newcommand{\vpsi}{\mbox{$\bm \psi$}}
\newcommand{\vphi}{\mbox{$\bm \phi$}}
\newcommand{\vxi}{\mbox{$\bm \xi$}}
\newcommand{\vth}{\mbox{$\bm \theta$}}
\newcommand{\vthh}{\mbox{$\bm {\hat \theta}$}}

\newcommand{\mgG}{\mbox{$\bm \Gamma$}}
\newcommand{\mgGh}{\mbox{$\hat {\bm \Gamma}$}}
\newcommand{\mgD}{\mbox{$\bm \Delta$}}
\newcommand{\mgU}{\mbox{$\bm \Upsilon$}}
\newcommand{\mgL}{\mbox{$\bm \Lambda$}}
\newcommand{\mgLh}{\mbox{$\bm {\hat \Lambda}$}}
\newcommand{\mPsi}{\mbox{$\bm \Psi$}}
\newcommand{\mgX}{\mbox{$\bm \Xi$}}
\newcommand{\mgS}{\mbox{$\bm \Sigma$}}

\newcommand{\mLambda}{\mbox{$\bm \Lambda$}}



%Abbreviatians for blackboard bold
\newcommand{\oA}{{\open A}}
\newcommand{\oC}{{\open C}}
\newcommand{\oF}{{\open F}}
\newcommand{\oN}{{\open N}}
\newcommand{\oP}{{\open P}}
\newcommand{\oQ}{{\open Q}}
\newcommand{\oR}{{\open R}}
\newcommand{\oZ}{{\open Z}}



\newcommand{\rH}{^{ \raisebox{1pt}{$\rm \scriptscriptstyle H$}}}
%\newcommand{\rH}{^{*}}
\newcommand{\rT}{^{ \raisebox{1.2pt}{$\rm \scriptstyle T$}}}
\newcommand{\rF}{_{ \raisebox{-1pt}{$\rm \scriptstyle F$}}}
\newcommand{\rE}{{\rm E}}




% mathematical environments
%\theoremstyle{plain}
\iffalse
    \newtheorem{theorem}{Theorem}[section]
    \newtheorem{lemma}[theorem]{Lemma}
    \newtheorem{principle}[theorem]{Principle}
    \newtheorem{prop}{Proposition}[section]
    \newtheorem{claim}{Claim}[section]

    %\theoremstyle{definition}
    \newtheorem{definition}{Definition}[section]
    %\theoremstyle{remark}
    \newtheorem{question}{Question}[section]
    \newtheorem{coro}{Corollary}[section]

    \newcommand{\proof}{Proof}
\fi


%\newcommand{\bds}{\begin {description}}
%\newcommand{\eds}{\end {description}}
\newcommand{\bds}{\begin {itemize}}
\newcommand{\eds}{\end {itemize}}
\newcommand{\bdf}{\begin{definition}}
\newcommand{\blm}{\begin{lemma}}
\newcommand{\edf}{\end{definition}}
\newcommand{\elm}{\end{lemma}}
\newcommand{\bthm}{\begin{theorem}}
\newcommand{\ethm}{\end{theorem}}
\newcommand{\bprp}{\begin{prop}}
\newcommand{\eprp}{\end{prop}}
\newcommand{\bcl}{\begin{claim}}
\newcommand{\ecl}{\end{claim}}
\newcommand{\bcr}{\begin{coro}}
\newcommand{\ecr}{\end{coro}}
\newcommand{\bquest}{\begin{question}}
\newcommand{\equest}{\end{question}}

%Abbreviatians for other symbols
\newcommand{\rarrow}{{\rightarrow}}
\newcommand{\Rarrow}{{\Rightarrow}}
\newcommand{\larrow}{{\larrow}}
\newcommand{\Larrow}{{\Leftarrow}}
\newcommand{\restrict}{{\upharpoonright}}
\newcommand{\nin}{{\not \in}}





% Abrreviations
\newcommand{\ie}{\hbox{i.e., }}
\newcommand{\eg}{\hbox{e.g., }}
\newcommand{\etal}{\hbox{et al.}}
\newcommand{\cf}{\hbox{cf.\ }}
\newcommand{\viz}{\hbox{viz.\ }}
\newcommand{\ao}{\hbox{a.o.\ }}


% mathematical functions and constants
\def\Re{\ensuremath{\hbox{Re}}}
\def\Im{\ensuremath{\hbox{Im}}}
\newcommand{\INR}{\ensuremath{\mathrm{INR}}}
\newcommand{\CRB}{\ensuremath{\mathrm{CRB}}}
\newcommand{\trace}{\ensuremath{\mathrm{tr}}}

\newcommand{\MDL}{\ensuremath{\mathrm{MDL}}}

\newcommand{\dom}{\ensuremath{\mathrm{dom}}}
\newcommand{\rng}{\ensuremath{\mathrm{rng}}}
\newcommand{\Span}{\ensuremath{\mathrm{span}}}
\newcommand{\On}{\ensuremath{\mathrm{On}}}
\newcommand{\otp}{\ensuremath{\mathrm{otp}}}
\newcommand{\ZFC}{\ensuremath{\mathrm{ZFC}}}
\newcommand{\argmin}{\ensuremath{\mathrm{arg}\min}}
\newcommand{\argmax}{\ensuremath{\mathrm{arg}\max}}
\newcommand{\kernel}{\ensuremath{\mathrm{ker}}}
\newcommand{\Ran}{\ensuremath{\mathrm{ran}}}	% gebruik Ran en Ker voor X_2
\newcommand{\ran}{\ensuremath{\mathrm{ran}}}	% gebruik Ran en Ker voor X_2
\newcommand{\Ker}{\ensuremath{\mathrm{ker}}}
\newcommand{\clr}{\ensuremath{\mathrm{cl}}}	% closure
\newcommand{\uestable}{u.e.\ stable}



%Abbreviatians for caligraphic letters

\newcommand{\Nu}{{\cal V}}
\newcommand{\cA}{{\ensuremath{\mathcal{A}}}}
\newcommand{\cB}{{\ensuremath{\mathcal{B}}}}
\newcommand{\cC}{{\ensuremath{\mathcal{C}}}}
\newcommand{\cD}{{\ensuremath{\mathcal{D}}}}
\newcommand{\cE}{{\ensuremath{\mathcal{E}}}}
\newcommand{\cF}{{\ensuremath{\mathcal{F}}}}
\newcommand{\cG}{{\ensuremath{\mathcal{G}}}}
\newcommand{\cH}{{\ensuremath{\mathcal{H}}}}
\newcommand{\cI}{{\ensuremath{\mathcal{I}}}}
\newcommand{\cJ}{{\ensuremath{\mathcal{J}}}}
\newcommand{\cK}{{\ensuremath{\mathcal{K}}}}
\newcommand{\cL}{{\ensuremath{\mathcal{L}}}}
\newcommand{\cM}{{\ensuremath{\mathcal{M}}}}
\newcommand{\cN}{{\ensuremath{\mathcal{N}}}}
\newcommand{\cO}{{\ensuremath{\mathcal{O}}}}
\newcommand{\cP}{{\ensuremath{\mathcal{P}}}}
\newcommand{\cQ}{{\ensuremath{\mathcal{Q}}}}
\newcommand{\cR}{{\ensuremath{\mathcal{R}}}}
\newcommand{\cS}{{\ensuremath{\mathcal{S}}}}
\newcommand{\cT}{{\ensuremath{\mathcal{T}}}}
\newcommand{\cU}{{\ensuremath{\mathcal{U}}}}
\newcommand{\cV}{{\ensuremath{\mathcal{V}}}}
\newcommand{\cW}{{\ensuremath{\mathcal{W}}}}
\newcommand{\cX}{{\ensuremath{\mathcal{X}}}}
\newcommand{\cY}{{\ensuremath{\mathcal{Y}}}}
\newcommand{\cZ}{{\ensuremath{\mathcal{Z}}}}

\newcommand{\coA}{{\ensuremath{\overline{\mathcal{A}}}}}
\newcommand{\coB}{{\ensuremath{\overline{\mathcal{B}}}}}
\newcommand{\coH}{{\ensuremath{\overline{\mathcal{H}}}}}



\newcommand{\Ht}{{\ensuremath{\tilde{H}}}}
\newcommand{\Nt}{{\ensuremath{\tilde{N}}}}
\newcommand{\Tp}{{\ensuremath{\tilde{\Theta}}}}
\newcommand{\tp}{{\ensuremath{\tilde{\theta}}}}
\newcommand{\Jp}{{\ensuremath{\tilde{J}}}}
\newcommand{\jp}{{\ensuremath{\tilde{j}}}}


% abbreviations for bold english letters (vectors)

\newcommand{\va}{{\ensuremath{{\mathbf{a}}}}}
\newcommand{\vah}{{\ensuremath{{\mathbf{\hat{a}}}}}}
\newcommand{\vat}{{\ensuremath{{\mathbf{\tilde{a}}}}}}
\newcommand{\vb}{{\ensuremath{{\mathbf{b}}}}}
\newcommand{\vc}{{\ensuremath{{\mathbf{c}}}}}
\newcommand{\vd}{{\ensuremath{{\mathbf{d}}}}}
\newcommand{\ve}{{\ensuremath{{\mathbf{e}}}}}
\newcommand{\vk}{{\ensuremath{{\mathbf{k}}}}}
\newcommand{\vf}{{\ensuremath{{\mathbf{f}}}}}
\newcommand{\vg}{{\ensuremath{{\mathbf{g}}}}}
\newcommand{\vgh}{{\ensuremath{{\mathbf{\hat{g}}}}}}
\newcommand{\vl}{{\ensuremath{{\mathbf{l}}}}}
\newcommand{\vm}{{\ensuremath{{\mathbf{m}}}}}
\newcommand{\vh}{{\ensuremath{{\mathbf{h}}}}}
\newcommand{\vhh}{{\ensuremath{{\mathbf{\hat{h}}}}}}
\newcommand{\vn}{{\ensuremath{{\mathbf{n}}}}}
\newcommand{\vnt}{{\ensuremath{{\mathbf{\tilde{n}}}}}}
\newcommand{\vq}{{\ensuremath{{\mathbf{q}}}}}
\newcommand{\vr}{{\ensuremath{{\mathbf{r}}}}}
\newcommand{\vs}{{\ensuremath{{\mathbf{s}}}}}
\newcommand{\vsh}{{\ensuremath{{\mathbf{\hat{s}}}}}}
\newcommand{\vst}{{\ensuremath{{\mathbf{\tilde{s}}}}}}
\newcommand{\vt}{{\ensuremath{{\mathbf{t}}}}}
\newcommand{\vu}{{\ensuremath{{\mathbf{u}}}}}
\newcommand{\vv}{{\ensuremath{{\mathbf{v}}}}}
\newcommand{\vvh}{{\ensuremath{{\mathbf{\hat{v}}}}}}
\newcommand{\vw}{{\ensuremath{{\mathbf{w}}}}}
\newcommand{\vwh}{{\ensuremath{{\mathbf{\hat{w}}}}}}
\newcommand{\wt}{{\ensuremath{{{\tilde{w}}}}}}
\newcommand{\vwt}{{\ensuremath{{\mathbf{\tilde{w}}}}}}
\newcommand{\vx}{{\ensuremath{{\mathbf{x}}}}}
\newcommand{\vxh}{{\ensuremath{{\mathbf{\hat{x}}}}}}
\newcommand{\vxt}{{\ensuremath{{\mathbf{\tilde{x}}}}}}
\newcommand{\vy}{{\ensuremath{{\mathbf{y}}}}}
\newcommand{\vz}{{\ensuremath{{\mathbf{z}}}}}

\newcommand{\vzero}{{\ensuremath{{\mathbf{0}}}}}
\newcommand{\vone}{{\ensuremath{{\mathbf{1}}}}}


% abbreviations for matrices
\newcommand{\mA}{{\ensuremath{\mathbf{A}}}}
\newcommand{\mAh}{{\ensuremath{\mathbf{\hat{A}}}}}
\newcommand{\mAt}{{\ensuremath{\mathbf{\tilde{A}}}}}
\newcommand{\mB}{{\ensuremath{\mathbf{B}}}}
\newcommand{\mBh}{{\ensuremath{\mathbf{\hat{B}}}}}
\newcommand{\mC}{{\ensuremath{\mathbf{C}}}}
\newcommand{\mCh}{{\ensuremath{\mathbf{\hat{C}}}}}
\newcommand{\mD}{{\ensuremath{\mathbf{D}}}}
\newcommand{\mDt}{{\ensuremath{\mathbf{\tilde{D}}}}}
\newcommand{\mDh}{{\ensuremath{\mathbf{\hat{D}}}}}
\newcommand{\mE}{{\ensuremath{\mathbf{E}}}}
\newcommand{\mF}{{\ensuremath{\mathbf{F}}}}
\newcommand{\mG}{{\ensuremath{\mathbf{G}}}}
\newcommand{\mH}{{\ensuremath{\mathbf{H}}}}
\newcommand{\mHb}{{\ensuremath{\mathbf{\bar{H}}}}}
\newcommand{\mI}{{\ensuremath{\mathbf{I}}}}
\newcommand{\mIh}{{\ensuremath{\mathbf{\hat{I}}}}}
\newcommand{\mJ}{{\ensuremath{\mathbf{J}}}}
\newcommand{\mL}{{\ensuremath{\mathbf{L}}}}
\newcommand{\mLb}{{\ensuremath{\mathbf{\bar{L}}}}}
\newcommand{\mM}{{\ensuremath{\mathbf{M}}}}
\newcommand{\mMh}{{\ensuremath{\mathbf{\hat{M}}}}}
\newcommand{\mN}{{\ensuremath{\mathbf{N}}}}
\newcommand{\mP}{{\ensuremath{\mathbf{P}}}}
\newcommand{\mQ}{{\ensuremath{\mathbf{Q}}}}
\newcommand{\mQh}{{\ensuremath{\mathbf{\hat{Q}}}}}
\newcommand{\mR}{{\ensuremath{\mathbf{R}}}}
\newcommand{\mRh}{{\ensuremath{\mathbf{\hat{R}}}}}
\newcommand{\mRt}{{\ensuremath{\mathbf{\tilde{R}}}}}
\newcommand{\mS}{{\ensuremath{\mathbf{S}}}}
\newcommand{\mSb}{{\ensuremath{\mathbf{\bar{S}}}}}
\newcommand{\mSh}{{\ensuremath{\mathbf{\hat{S}}}}}
\newcommand{\mSt}{{\ensuremath{\mathbf{\tilde{S}}}}}
\newcommand{\mT}{{\ensuremath{\mathbf{T}}}}
\newcommand{\mU}{{\ensuremath{\mathbf{U}}}}
\newcommand{\mUh}{{\ensuremath{\mathbf{\hat{U}}}}}
\newcommand{\mV}{{\ensuremath{\mathbf{V}}}}
\newcommand{\mVh}{{\ensuremath{\mathbf{\hat{V}}}}}
\newcommand{\mW}{{\ensuremath{\mathbf{W}}}}
\newcommand{\mWh}{{\ensuremath{\mathbf{\hat{W}}}}}
\newcommand{\mWt}{{\ensuremath{\mathbf{\tilde{W}}}}}
\newcommand{\mX}{{\ensuremath{\mathbf{X}}}}
\newcommand{\mY}{{\ensuremath{\mathbf{Y}}}}
\newcommand{\mZ}{{\ensuremath{\mathbf{Z}}}}


\newcommand{\Ah}{{\ensuremath{\hat{A}}}}
\newcommand{\Bh}{{\ensuremath{\hat{B}}}}
\newcommand{\bAh}{{\ensuremath{\hat{\mathbf{A}}}}}
\newcommand{\bDh}{{\ensuremath{\hat{\mathbf{D}}}}}
\newcommand{\bRh}{{\ensuremath{\hat{\mathbf{R}}}}}
\newcommand{\bUh}{{\ensuremath{\hat{\mathbf{U}}}}}
\newcommand{\bUc}{{\ensuremath{\underline{\mathbf{U}}}}}
\newcommand{\bLambdah}{{\ensuremath{\hat{\bLambda}}}}
\newcommand{\byh}{{\ensuremath{\hat{\mathbf y}}}}




\newcommand{\Mp}{{\ensuremath{M^\prime}}}
\newcommand{\Kp}{{\ensuremath{K^\prime}}}
\newcommand{\KpH}{{\ensuremath{K^{\prime *}}}}
\newcommand{\bPL}{{\ensuremath{\mathbf P^\prime}}}







%  []
% \def\qed{\hfill {$\Box$}}
% The tex-book p.106: adapted `signed' macro to ensure qed always at end of line
\usepackage{latexsym}
\def\qed{{\unskip\nobreak\hfil\penalty50
    \hskip2em\hbox{}\nobreak\hfil{$\Box$}\parfillskip=0pt 
    \vspace{1ex plus 2pt}\par}}



\def\IC{\mathbb C}
\def\IN{\mathbb N}
\def\IZ{\mathbb Z}
\def\IR{\mathbb R}
\def\IQ{\mathbb Q}

\iffalse
    % The set of complex numbers
    \def\IC{{
       \mathord{
	  \hbox to 0em{
	     \hskip-4pt
	     \ooalign{
	       \smash{\hskip1.9pt\raise2.6pt\hbox{$\scriptscriptstyle |$}}\crcr
	       \smash{\hbox{\rm\sf C}} }
	     \hidewidth}
	  \phantom{\hbox{\rm\sf C}}
    } }}
    % The set of natural numbers
    \def\IN{
	{\ooalign{
       \smash{\hskip2.2pt\raise1.5pt\hbox{$\scriptscriptstyle |$}}
       \vphantom{}\crcr
       \hbox{\rm\sf N}
	    }}
	    } 
    % The set of integers
    \def\IZ{
       {\ooalign{
       \smash{\hskip1.9pt\raise0pt\hbox{\rm\sf Z}}
       \vphantom{}\crcr
       \hbox{\rm\sf Z}
	    }}
	    } 
    % The set of reals
    \def\IR{
	{\ooalign{
       \smash{\hskip2.2pt\raise1.5pt\hbox{$\scriptscriptstyle |$}}
       \vphantom{}\crcr
       \smash{\hskip2.2pt\raise3.3pt\hbox{$\scriptscriptstyle |$}}
       \vphantom{}\crcr
       \hbox{\rm\sf R}
	    }}
	    } 
\fi



% from AMSTEX \sphat
\def\shat{^{\mathchoice{}{}%
 {\,\,\smash{\hbox{\lower4pt\hbox{$\widehat{\null}$}}}}%
 {\,\smash{\hbox{\lower3pt\hbox{$\hat{\null}$}}}}}}

\def\lvec#1{\buildrel  \raisebox{-2.5pt}{$\scriptstyle \leftarrow$} \over #1 }

% hacks for bold \Sigma and \Theta

\def\bSigma{{
      \ooalign{
      \smash{\hskip.4pt\raise.4pt\hbox{$\Sigma$}}\vphantom{}\crcr
      \smash{\hskip.7pt\raise.6pt\hbox{$\Sigma$}}\vphantom{}\crcr
      \smash{\hbox{$\Sigma$}}\vphantom{$\Sigma$}}
      \vphantom{\hbox{$\Sigma$}}
      }}
\def\bTheta{{
      \ooalign{
      \smash{\hskip.5pt\raise.5pt\hbox{$\Theta$}}\vphantom{}\crcr
      \smash{\hskip.0pt\raise.1pt\hbox{$\Theta$}}\vphantom{}\crcr
      \smash{\hbox{$\Theta$}}\vphantom{$\Theta$}}
      \vphantom{\hbox{$\Theta$}}
      }}
\def\bDelta{{
      \ooalign{
      \smash{\hskip.4pt\raise.4pt\hbox{$\Delta$}}\vphantom{}\crcr
      \smash{\hskip.7pt\raise.6pt\hbox{$\Delta$}}\vphantom{}\crcr
      \smash{\hbox{$\Delta$}}\vphantom{$\Delta$}}
      \vphantom{\hbox{$\Delta$}}
      }}
\def\bLambda{{
      \ooalign{
      \smash{\hskip.5pt\raise.5pt\hbox{$\Lambda$}}\vphantom{}\crcr
      \smash{\hskip.0pt\raise.1pt\hbox{$\Lambda$}}\vphantom{}\crcr
      \smash{\hbox{$\Lambda$}}\vphantom{$\Lambda$}}
      \vphantom{\hbox{$\Lambda$}}
      }}



% Bordermatrices with square brackets [] iso ()
\makeatletter
\def\pmatrix#1{\left[\matrix{#1}\right]}
\def\bordermatrix#1{\begingroup \m@th
  \@tempdima 8.75\p@
  \setbox\z@\vbox{%
    \def\cr{\crcr\noalign{\kern2\p@\global\let\cr\endline}}%
    \ialign{$##$\hfil\kern2\p@\kern\@tempdima&\thinspace\hfil$##$\hfil
      &&\quad\hfil$##$\hfil\crcr
      \omit\strut\hfil\crcr\noalign{\kern-\baselineskip}%
      #1\crcr\omit\strut\cr}}%
  \setbox\tw@\vbox{\unvcopy\z@\global\setbox\@ne\lastbox}%
  \setbox\tw@\hbox{\unhbox\@ne\unskip\global\setbox\@ne\lastbox}%
  \setbox\tw@\hbox{$\kern\wd\@ne\kern-\@tempdima\left[\kern-\wd\@ne
    \global\setbox\@ne\vbox{\box\@ne\kern2\p@}%
    \vcenter{\kern-\ht\@ne\unvbox\z@\kern-\baselineskip}\,\right]$}%
  \null\;\vbox{\kern\ht\@ne\box\tw@}\endgroup}
\makeatother



%
\def\dashlist{\list{\mbox{--}}{\topsep 5pt plus .25pt
    \itemsep 5pt \parsep 0.3ex plus .25pt
    \labelwidth 12pt \itemindent 0pt \labelsep 3pt \listparindent 0pt
    \leftmargin 15pt }}
    \let\enddashlist\endlist
%
\newcommand{\vgc}{{\ensuremath{\mathbf{\bar{g}}}}}
\newcommand{\mXh}{{\ensuremath{\mathbf{\hat{X}}}}}

\makeatletter
\def\argmin{\mathop{\operator@font arg\,min}}
\def\argmax{\mathop{\operator@font arg\,max}}
\makeatother

\newcommand{\dr}{\mbox{d}}

\newcommand{\half}{\frac{1}{2}}
\newcommand{\CM}{{\cC\!\cM}}
\newcommand{\ZCM}{{\mbox{ZCM}}}
\newcommand{\Rp}{{R^\prime}}
\newcommand{\Rpp}{{R^{\prime \prime}}}
\newcommand{\dist}{\mbox{\rm dist}}
\newcommand{\SINR}{{\mbox{SINR}}}
\newcommand{\SNR}{{\mbox{SNR}}}
\newcommand{\sinr}{{\mbox{sinr}}}
\newcommand{\SIR}{{\mbox{SIR}}}
\newcommand{\sir}{{\mbox{sir}}}

\newcommand{\var}{\mbox{\rm var}}
\newcommand{\cum}{\mbox{\rm cum}}
\newcommand{\real}{\mbox{\rm real}}
\newcommand{\imag}{\mbox{\rm imag}}
\renewcommand{\Re}{\mbox{\rm Re}}
\renewcommand{\Im}{\mbox{\rm Im}}
\newcommand{\eig}{\mbox{\rm eig}}
\newcommand{\diag}{\mbox{\rm diag}}
\newcommand{\spann}{\mbox{\rm span}}
\newcommand{\rank}{\mbox{\rm rank}}
\newcommand{\Null}{\mbox{\rm Null}}
%\newcommand{\argmin}{\mbox{\rm arg}\min}
\newcommand{\Tr}{\mbox{\rm Tr}}
\newcommand{\tr}{\mbox{\rm tr}}
\newcommand{\dimm}{\mbox{\rm dim }}
\newcommand{\sdim}{\mbox{\rm s-dim }}
\newcommand{\vect}{\mbox{\rm vec}}
\newcommand{\rvec}{\mbox{\rm vecr}}
\newcommand{\unvect}{{\vect}^{-1}}
\newcommand{\vech}{\mbox{\rm vech}}
\newcommand{\unvech}{{\vech}^{-1}}
\newcommand{\range}{\mbox{\rm ran}}
\def\expect#1{\mbox{\rm E}\{#1\}}
\newcommand{\unvec}{\mbox{\rm vec}^{-1}}
\newcommand{\row}{\mbox{\rm row}}
\newcommand{\col}{\mbox{\rm col}}
\newcommand{\cov}{\mbox{\rm cov}}
\newcommand{\sign}{\mbox{\rm sign}}
\newcommand{\cond}{\mbox{\rm cond}}
\newcommand{\suchthat}{\hspace{1cm}\mbox{\rm s.t.}\hspace{.5cm}}
\newcommand{\GE}{{\rm GE}}

\newcommand{\fracN}{\textstyle\frac{1}{N}}

\def\cf{{cf.\ }}
\def\viz{{viz.\ }}
\def\etal{{et al.\ }}
\def\eg{{e.g.,\ }}
\def\ie{{i.e.,\ }}

\def\bm#1{\mbox{\boldmath $#1$}}
\newcommand{\balpha}{{\bm\alpha}}
\newcommand{\btau}{{\bm\tau}}
\newcommand{\bbeta}{{\bm\beta}}
\newcommand{\blambda}{{\bm\lambda}}
\newcommand{\btheta}{{\bm\theta}}

\newcommand{\bea}{\begin{array}}
\newcommand{\ena}{\end{array}}
%
\newcommand{\beq}{\begin{equation}}
\newcommand{\enq}{\end{equation}}

\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\enqa}{\end{eqnarray}}

\newcommand{\beqan}{\begin{eqnarray*}}
\newcommand{\enqan}{\end{eqnarray*}}

\newcommand{\AL}{\begin{enumerate}}
\newcommand{\ALE}{\end{enumerate}}





\newcommand{\Vn}{\Va^{\perp}}
\newcommand{\Un}{\Ua^{\perp}}
\newcommand{\bVn}{\bVa^{\perp}}
\newcommand{\bUn}{\bUa^{\perp}}
%\newcommand{\VnH}{\Va^{\perp{\rm\scriptscriptstyle *}}}
%\newcommand{\UnH}{\Ua^{\perp{\rm\scriptscriptstyle *}}}
\newcommand{\VnH}{\Va^{\perp *}}
\newcommand{\bVnH}{\bVa^{\perp *}}
\newcommand{\UnH}{\Ua^{\perp *}}
\newcommand{\bUnH}{\bUa^{\perp *}}
\newcommand{\sk}{\sigma_{d+1}}
\newcommand{\vk}{\bv_{d+1}}
\newcommand{\uk}{\bu_{d+1}}
\newcommand{\ukz}{u_{d+1}(z)}
\newcommand{\Ls}{\Lambda_s}
\newcommand{\Ln}{\Lambda_n}
\newcommand{\Lo}{\tilde{\Lambda}}
\newcommand{\Loh}{\tilde{\Lambda}^{1/2}}
\newcommand{\Las}{\hat{\Lambda}_s}
\newcommand{\Wh}{W^{1/2}}
\newcommand{\Wopt}{W_{\mbox{\scriptsize opt}}}
\newcommand{\Wlo}{W_{1,\mbox{\scriptsize opt}}}
 

% anti-diagonal dots
\def\addots{\mathinner{
    \mkern1mu\raise0pt\vbox{\kern7pt\hbox{.}}
    \mkern2mu\raise4pt\hbox{.}
    \mkern2mu\raise7pt\hbox{.}
    \mkern1mu}}

% steep diagonal dots
\def\sddots{\mathinner{
    \mkern.8mu\raise7pt\hbox{.}
    \mkern.8mu\raise4pt\hbox{.}
    \mkern.8mu\raise0pt\vbox{\kern7pt\hbox{.}}
    \mkern1mu}}

% steep anti-diagonal dots
\def\saddots{\mathinner{
    \mkern.2mu\raise0pt\vbox{\kern7pt\hbox{.}}
    \mkern.2mu\raise4pt\hbox{.}
    \mkern.2mu\raise7pt\hbox{.}
    \mkern1mu}}


\newcommand{\cHt}{{\tilde{\cal H}}}


\newcommand{\ba}{{\ensuremath{\mathbf{a}}}}
\newcommand{\bb}{{\ensuremath{\mathbf{b}}}}
\newcommand{\bfb}{{\ensuremath{\mathbf{b}}}}
\newcommand{\bc}{{\ensuremath{\mathbf{c}}}}
\newcommand{\bd}{{\ensuremath{\mathbf{d}}}}
\newcommand{\be}{{\ensuremath{\mathbf{e}}}}
\newcommand{\bff}{{\ensuremath{\mathbf{f}}}}
\newcommand{\bg}{{\ensuremath{\mathbf{g}}}}
\newcommand{\bh}{{\ensuremath{\mathbf{h}}}}
\newcommand{\bi}{{\ensuremath{\mathbf{i}}}}
\newcommand{\bfm}{{\ensuremath{\mathbf{m}}}}
\newcommand{\bn}{{\ensuremath{\mathbf{n}}}}
\newcommand{\bp}{{\ensuremath{\mathbf{p}}}}
\newcommand{\bq}{{\ensuremath{\mathbf{q}}}}
\newcommand{\br}{{\ensuremath{\mathbf{r}}}}
\newcommand{\bs}{{\ensuremath{\mathbf{s}}}}
\newcommand{\bt}{{\ensuremath{\mathbf{t}}}}
\newcommand{\bu}{{\ensuremath{\mathbf{u}}}}
\newcommand{\bv}{{\ensuremath{\mathbf{v}}}}
\newcommand{\bw}{{\ensuremath{\mathbf{w}}}}
\newcommand{\bx}{{\ensuremath{\mathbf{x}}}}
\newcommand{\by}{{\ensuremath{\mathbf{y}}}}
\newcommand{\bz}{{\ensuremath{\mathbf{z}}}}

\newcommand{\bA}{{\ensuremath{\mathbf{A}}}}
\newcommand{\bB}{{\ensuremath{\mathbf{B}}}}
\newcommand{\bC}{{\ensuremath{\mathbf{C}}}}
\newcommand{\bD}{{\ensuremath{\mathbf{D}}}}
\newcommand{\bE}{{\ensuremath{\mathbf{E}}}}
\newcommand{\bF}{{\ensuremath{\mathbf{F}}}}
\newcommand{\bG}{{\ensuremath{\mathbf{G}}}}
\newcommand{\bH}{{\ensuremath{\mathbf{H}}}}
\newcommand{\bI}{{\ensuremath{\mathbf{I}}}}
\newcommand{\bJ}{{\ensuremath{\mathbf{J}}}}
\newcommand{\bK}{{\ensuremath{\mathbf{K}}}}
\newcommand{\bL}{{\ensuremath{\mathbf{L}}}}
\newcommand{\bM}{{\ensuremath{\mathbf{M}}}}
\newcommand{\bN}{{\ensuremath{\mathbf{N}}}}
\newcommand{\bO}{{\ensuremath{\mathbf{O}}}}
\newcommand{\bP}{{\ensuremath{\mathbf{P}}}}
\newcommand{\bQ}{{\ensuremath{\mathbf{Q}}}}
\newcommand{\bR}{{\ensuremath{\mathbf{R}}}}
\newcommand{\bS}{{\ensuremath{\mathbf{S}}}}
\newcommand{\bT}{{\ensuremath{\mathbf{T}}}}
\newcommand{\bU}{{\ensuremath{\mathbf{U}}}}
\newcommand{\bV}{{\ensuremath{\mathbf{V}}}}
\newcommand{\bW}{{\ensuremath{\mathbf{W}}}}
\newcommand{\bX}{{\ensuremath{\mathbf{X}}}}
\newcommand{\bY}{{\ensuremath{\mathbf{Y}}}}
\newcommand{\bZ}{{\ensuremath{\mathbf{Z}}}}


\newcommand{\bthetaa}{\hat{{\btheta}}}

\newcommand{\da}{\hat{{\bf d}}}
\newcommand{\sa}{\hat{{\bf s}}}
\newcommand{\ea}{\hat{{\bf e}}}
\newcommand{\xa}{\hat{{x}}}
\newcommand{\ya}{\hat{{\bf y}}}

\newcommand{\bpa}{{\ensuremath{\mathbf{\hat{p}}}}}

\newcommand{\Aa}{\hat{A}}
\newcommand{\Ca}{\hat{C}}
\newcommand{\Ea}{\hat{E}}
\newcommand{\Ha}{\hat{H}}
\newcommand{\Lah}{\hat{\Lambda}}
\newcommand{\Ma}{\hat{M}}
\newcommand{\Na}{\hat{N}}
\newcommand{\Pa}{\hat{P}}
\newcommand{\Qa}{\hat{Q}}
\newcommand{\Ra}{\hat{R}}
\newcommand{\Sa}{\hat{\Sigma}}
\newcommand{\Sn}{\hat{\Sigma}^\perp}
\newcommand{\Ta}{\hat{T}}
\newcommand{\Ua}{\hat{U}}
\newcommand{\Va}{\hat{V}}
\newcommand{\Xa}{\hat{X}}
\newcommand{\Ya}{\hat{Y}}
\newcommand{\Za}{\hat{Z}}

\newcommand{\baa}{{\ensuremath{\mathbf{\hat{a}}}}}
\newcommand{\bta}{{\ensuremath{\mathbf{\hat{t}}}}}

\newcommand{\bAa}{{\ensuremath{\mathbf{\hat{A}}}}}
\newcommand{\bCa}{{\ensuremath{\mathbf{\hat{C}}}}}
\newcommand{\bDa}{{\ensuremath{\mathbf{\hat{D}}}}}
\newcommand{\bEa}{{\ensuremath{\mathbf{\hat{E}}}}}
\newcommand{\bEaw}{{\ensuremath{\mathbf{\underline{\hat{E}}}}}}
\newcommand{\bHa}{{\ensuremath{\mathbf{\hat{H}}}}}
\newcommand{\bKa}{{\ensuremath{\mathbf{\hat{K}}}}}
\newcommand{\bLah}{{\hat{\bLambda}}}
\newcommand{\bMa}{{\ensuremath{\mathbf{\hat{M}}}}}
\newcommand{\bNa}{{\ensuremath{\mathbf{\hat{N}}}}}
\newcommand{\bPa}{{\ensuremath{\mathbf{\hat{P}}}}}
\newcommand{\bQa}{{\ensuremath{\mathbf{\hat{Q}}}}}
\newcommand{\bRa}{{\ensuremath{\mathbf{\hat{R}}}}}
\newcommand{\bSigmah}{\hat{\bSigma}}
\newcommand{\bSn}{{{\bSigma}^\perp}}
\newcommand{\bTa}{{\ensuremath{\mathbf{\hat{T}}}}}
\newcommand{\bUa}{{\ensuremath{\mathbf{\hat{U}}}}}
\newcommand{\bVa}{{\ensuremath{\mathbf{\hat{V}}}}}
\newcommand{\bXa}{{\ensuremath{\mathbf{\hat{X}}}}}
\newcommand{\bWa}{{\ensuremath{\mathbf{\hat{W}}}}}
\newcommand{\bYa}{{\ensuremath{\mathbf{\hat{Y}}}}}
\newcommand{\bZa}{{\ensuremath{\mathbf{\hat{Z}}}}}

% bar denotes conjugate
% tilde denotes noise
\newcommand{\Ac}{\bar{A}}
\newcommand{\Vc}{\bar{V}}
\newcommand{\Wc}{\bar{W}}
\newcommand{\Xtc}{\bar{\tilde{X}}}
\newcommand{\btc}{\bar{{\bf t}}}
\newcommand{\bat}{\tilde{{\bf a}}}
\newcommand{\bxt}{\tilde{{\bf x}}}
\newcommand{\bpt}{\tilde{{\bf p}}}
\newcommand{\xt}{\tilde{{\bf x}}}
\newcommand{\xtc}{\bar{\tilde{{\bf x}}}}
\newcommand{\Gt}{\tilde{G}}
\newcommand{\Pt}{\tilde{P}}
\newcommand{\Kt}{\tilde{K}}
\newcommand{\Xt}{\tilde{X}}
\newcommand{\Rt}{\tilde{R}}
\newcommand{\Ct}{\tilde{C}}
\newcommand{\Et}{\tilde{E}}

\newcommand{\bAc}{{\ensuremath{\mathbf{\bar{A}}}}}
\newcommand{\bDc}{{\ensuremath{\mathbf{\bar{D}}}}}
\newcommand{\bTc}{{\ensuremath{\mathbf{\bar{T}}}}}
\newcommand{\bRc}{{\ensuremath{\mathbf{\bar{R}}}}}
\newcommand{\bVc}{{\ensuremath{\mathbf{\bar{V}}}}}
\newcommand{\bWc}{{\ensuremath{\mathbf{\bar{W}}}}}

\newcommand{\bCt}{{\ensuremath{\mathbf{\tilde{C}}}}}
\newcommand{\bEt}{{\ensuremath{\mathbf{\tilde{E}}}}}
\newcommand{\bGt}{{\ensuremath{\mathbf{\tilde{G}}}}}
\newcommand{\bKt}{{\ensuremath{\mathbf{\tilde{K}}}}}
\newcommand{\bPt}{{\ensuremath{\mathbf{\tilde{P}}}}}
\newcommand{\bRt}{{\ensuremath{\mathbf{\tilde{R}}}}}
\newcommand{\bXt}{{\ensuremath{\mathbf{\tilde{X}}}}}

\newcommand{\bXtc}{{\ensuremath{\mathbf{\bar{\tilde{X}}}}}}

\newcommand{\Xac}{\bar{\hat{X}}}
\newcommand{\Xc}{\bar{X}}
\newcommand{\bXac}{{\mathbf{\bar{\hat{X}}}}}
\newcommand{\bXc}{{\mathbf{\bar{X}}}}
\newcommand{\bxc}{\bar{\bf x}}
\newcommand{\bec}{\bar{\bf e}}

\def\bac{\bar{\ba}}
\def\bxc{\bar{\bx}}
\def\bwc{\bar{\bw}}
\def\bwt{\tilde{\bw}}
\def\bst{\tilde{\bs}}
\def\bsc{\bar{\bs}}

% whitened denoted by underline
\def\baw{\underline{\ba}}
\def\bacw{\underline{\bac}}
\def\baww{\underline{\underline{\ba}}}
\def\bacww{\underline{\underline{\bac}}}
\def\Aw{\underline{A}}
\def\Acw{\underline{\Ac}}
\def\Cw{\underline{C}}
\def\Ctw{\underline{\Ct}}
\def\Nw{\underline{N}}
\def\Gw{\underline{G}}
\def\Pw{\underline{P}}
\def\Rw{\underline{R}}
\def\Ww{\underline{W}}
\def\Xw{\underline{X}}
\def\Xtw{\underline{\Xt}}
\def\bxtw{\underline{\bxt}}
\def\xtw{\underline{\bxt}}
\def\baw{\underline{\ba}}
\def\bxw{\underline{\bx}}
\def\bxcw{\underline{\bxc}}
\def\bww{\underline{\bw}}
\def\byw{\underline{\by}}
\def\Xww{\underline{\underline{X}}}
\def\Xtww{\underline{\underline{\Xt}}}
\def\Ctww{\underline{\underline{\Ct}}}
\def\Aww{\underline{\underline{A}}}
\def\Acww{\underline{\underline{\Ac}}}
\def\Nww{\underline{\underline{N}}}
\def\Rtww{\underline{\underline{\Rt}}}
\def\Ktww{\underline{\underline{\Kt}}}
\def\Kww{\underline{\underline{K}}}

\def\bAw{\underline{\bA}}
\def\bAcw{\underline{\bAc}}
\def\bCw{\underline{\bC}}
\def\bCtw{\underline{\bCt}}
\def\bCaw{\underline{\bCa}}
\def\bNw{\underline{\bN}}
\def\bGw{\underline{\bG}}
\def\bPw{\underline{\bP}}
\def\bRw{\underline{\bR}}
\def\bRaw{\underline{\bRa}}
\def\bWw{\underline{\bW}}
\def\bXw{\underline{\bX}}
\def\bXtw{\underline{\bXt}}
\def\bXww{\underline{\underline{\bX}}}
\def\bXtww{\underline{\underline{\bXt}}}
\def\bCtww{\underline{\underline{\bCt}}}
\def\bAww{\underline{\underline{\bA}}}
\def\bAcww{\underline{\underline{\bAc}}}
\def\bAaww{\underline{\underline{\bAa}}}
\def\bNww{\underline{\underline{\bN}}}
\def\bRtww{\underline{\underline{\bRt}}}
\def\bKtww{\underline{\underline{\bKt}}}
\def\bKaww{\underline{\underline{\bKa}}}
\def\bKww{\underline{\underline{\bK}}}

\def\bones{{\bf 1}}
\def\bzero{{\bf 0}}


\newcommand{\bXh}{{\hat{\bX}}}
\newcommand{\cHh}{{\hat{\cH}}}
\newcommand{\bQh}{{\hat{\bQ}}}

 

%  []
% \def\qed{\hfill {$\Box$}}
% The tex-book p.106: adapted `signed' macro to ensure qed always at end of line
\def\qed{{\unskip\nobreak\hfil\penalty50
    \hskip2em\hbox{}\nobreak\hfil{$\Box$}
    \parfillskip=0pt \vspace{2ex}\par}}

\newcommand{\nsimeq}{\stackrel { N}{\simeq} }

\newcommand{\sqperp}{^{[\perp]}}
\newcommand{\sqperpto}{{\mathbin{\;[\perp]\;}}}
%  [+] and [-]
\def\sqplus{\mathbin{
	{\ooalign{\hfil\raise.3ex\hbox{\scriptsize
	+}\hfil\crcr\mathhexbox274\crcr\mathhexbox275}}
	}} 
\def\sqminus{\mathbin{
	{\ooalign{\hfil\raise.3ex\hbox{\scriptsize
	--}\hfil\crcr\mathhexbox274\crcr\mathhexbox275}}
	}} 



% The set of complex numbers
\def\IC{{
   \mathord{
      \hbox to 0em{
	 \hskip-4pt
         \ooalign{
	   \smash{\hskip1.9pt\raise2.6pt\hbox{$\scriptscriptstyle |$}}\crcr
	   \smash{\hbox{\rm\sf C}} }
	 \hidewidth}
      \phantom{\hbox{\rm\sf C}}
} }}
% The set of natural numbers
\def\IN{
    {\ooalign{
   \smash{\hskip2.2pt\raise1.5pt\hbox{$\scriptscriptstyle |$}}\vphantom{}\crcr
   \hbox{\sf N}
	}}
	} 
% The set of integers
\def\IZ{
    {\ooalign{
   \smash{\hskip1.9pt\raise0pt\hbox{$\sf Z$}}\vphantom{}\crcr
   \hbox{\sf Z}
	}}
	} 
% The set of reals
\def\IR{
    {\ooalign{
   \smash{\hskip2.2pt\raise1.5pt\hbox{$\scriptscriptstyle |$}}\vphantom{}\crcr
   \smash{\hskip2.2pt\raise3.3pt\hbox{$\scriptscriptstyle |$}}\vphantom{}\crcr
   \hbox{\sf R}
	}}
	} 

% hacks for bold \Sigma and \Theta in TimesRoman: borrow from CM
\DeclareMathAlphabet{\mathcmb}{OT1}{cmr}{b}{n}

\def\bSigma{\ensuremath{\mathcmb{\Sigma}}}
\def\bLambda{\ensuremath{\mathcmb{\Lambda}}}
\def\bPi{\ensuremath{\mathcmb{\Pi}}}
\def\bTheta{\ensuremath{\mathcmb{\Theta}}}
\def\bGamma{\ensuremath{\mathcmb{\Gamma}}}

\def\bSa{\ensuremath{\mathcmb{\hat{\Sigma}}}}

\newcommand{\bPsi}{{\ensuremath{\mathcmb{\Psi}}}}
\newcommand{\bPsih}{{\ensuremath{\mathcmb{\hat{\Psi}}}}}


\def\bdot{{\scriptscriptstyle\bullet}}



% Indented 'list' 
% Usage: \SI
%          blabla
%        \EI

\def\indlist{\list{\mbox{}}{\topsep 0pt 
    \itemsep 5pt \parsep 0.3ex plus .25pt \parskip 0pt
    \labelwidth 20pt \itemindent 0pt \labelsep 2pt \listparindent 0pt
    \leftmargin 22pt }\item}
    \let\endindlist\endlist
\newcommand{\SI}{\begin{indlist}}
\newcommand{\EI}{\end{indlist}}



% Hanging indent after introline
% usage:
%    \hanglines{where\ }
%    $U$ is block lower and unitary,\\
%    $V$ is block upper and isometric, and\\
%    $T_0$ is upper with upper inverse.
%
\def\hanglines#1{
    \setbox1=\hbox{#1}%
    \hangindent=\wd1\hangafter=0
    \hskip -\hangindent
    \makebox[\hangindent]{\box1}\ignorespaces%
}

\def\dashlist{\list{\mbox{--}}{\topsep 5pt plus .25pt
    \itemsep 5pt \parsep 0.3ex plus .25pt
    \labelwidth 12pt \itemindent 0pt \labelsep 3pt \listparindent 0pt
    \leftmargin 15pt }}
    \let\enddashlist\endlist
%
\newcommand{\DL}{\begin{dashlist}}
\newcommand{\DLE}{\end{dashlist}}

% whitened denoted by underline
\def\baw{\underline{\ba}}
\def\bacw{\underline{\bac}}
\def\baww{\underline{\underline{\ba}}}
\def\bacww{\underline{\underline{\bac}}}
\def\Aw{\underline{A}}
\def\Acw{\underline{\Ac}}
\def\Cw{\underline{C}}
\def\Ctw{\underline{\Ct}}
\def\Nw{\underline{N}}
\def\Gw{\underline{G}}
\def\Pw{\underline{P}}
\def\Rw{\underline{R}}
\def\Ww{\underline{W}}
\def\Xw{\underline{X}}
\def\Xtw{\underline{\Xt}}
\def\bxtw{\underline{\bxt}}
\def\xtw{\underline{\bxt}}
\def\baw{\underline{\ba}}
\def\bxw{\underline{\bx}}
\def\bww{\underline{\bw}}
\def\byw{\underline{\by}}
\newcommand{\Gtw}{\underline{\Gt}}
\newcommand{\Ptw}{\underline{\Pt}}
\newcommand{\Rtw}{\underline{\Rt}}
\def\Xww{\underline{\underline{X}}}
\def\Xtww{\underline{\underline{\Xt}}}
\def\Ctww{\underline{\underline{\Ct}}}
\def\Aww{\underline{\underline{A}}}
\def\Acww{\underline{\underline{\Ac}}}
\def\Nww{\underline{\underline{N}}}
\def\Rtww{\underline{\underline{\Rt}}}
\def\Ktww{\underline{\underline{\Kt}}}
\def\Kww{\underline{\underline{K}}}

\def\bAw{\underline{\bA}}
\def\bAcw{\underline{\bAc}}
\def\bCw{\underline{\bC}}
\def\bCtw{\underline{\bCt}}
\def\bCaw{\underline{\bCa}}
\def\bNw{\underline{\bN}}
\def\bGw{\underline{\bG}}
\def\bPw{\underline{\bP}}
\def\bRw{\underline{\bR}}
\def\bWw{\underline{\bW}}
\def\bXw{\underline{\bX}}
\def\bXtw{\underline{\bXt}}
\def\bYw{\underline{\bY}}
\newcommand{\bGtw}{\underline{\bGt}}
\newcommand{\bPtw}{\underline{\bPt}}
\newcommand{\bRtw}{\underline{\bRt}}
\def\bXww{\underline{\underline{\bX}}}
\def\bXtww{\underline{\underline{\bXt}}}
\def\bCtww{\underline{\underline{\bCt}}}
\def\bAaw{\underline{\bAa}}
\def\bAww{\underline{\underline{\bA}}}
\def\bAcww{\underline{\underline{\bAc}}}
\def\bNww{\underline{\underline{\bN}}}
\def\bRtww{\underline{\underline{\bRt}}}
\def\bKtww{\underline{\underline{\bKt}}}
\def\bKww{\underline{\underline{\bK}}}

\newcommand{\Pap}{\bPv_{\bA}^\perp}
\newcommand{\Papt}{\bPv_{\bA(\btheta)}^\perp}

% composite denoted by undertilde
%\usepackage{amsmath}

% copied from amsmath: (don't load it all because destroys bold Sigma...)
\makeatletter
\def\setboxz@h{\setbox\z@\hbox}
\def\wdz@{\wd\z@}
\def\boxz@{\box\z@}
\def\underset#1#2{\binrel@{#2}%
  \binrel@@{\mathop{\kern\z@#2}\limits_{#1}}}
\def\binrel@#1{\begingroup
  \setboxz@h{\thinmuskip0mu
    \medmuskip\m@ne mu\thickmuskip\@ne mu
    \setbox\tw@\hbox{$#1\m@th$}\kern-\wd\tw@
    ${}#1{}\m@th$}%
  \edef\@tempa{\endgroup\let\noexpand\binrel@@
    \ifdim\wdz@<\z@ \mathbin
    \else\ifdim\wdz@>\z@ \mathrel
    \else \relax\fi\fi}%
  \@tempa
}
\let\binrel@@\relax%
\makeatother

% best choice:
\def\undertilde#1{\smash{\underset{^{\mbox{\~{}}}}{#1}}\vphantom{#1}}

\newcommand{\Av}{\ensuremath{\undertilde{A}}}
\newcommand{\bAv}{\ensuremath{\mathbf{\undertilde{\bA}}}}
\newcommand{\Dv}{\ensuremath{\undertilde{D}}}
\newcommand{\bDv}{\ensuremath{\mathbf{\undertilde{\bD}}}}
\newcommand{\bPv}{\ensuremath{\mathbf{\undertilde{\bP}}}}
\newcommand{\Uv}{\ensuremath{\undertilde{U}}}
\newcommand{\bUv}{\ensuremath{\mathbf{\undertilde{\bU}}}}
\newcommand{\bUva}{\ensuremath{\mathbf{\undertilde{\bUa}}}}
\newcommand{\bLvah}{\ensuremath{\mathbf{\undertilde{\bLah}}}}
\newcommand{\bVv}{\ensuremath{\mathbf{\undertilde{\bV}}}}
\newcommand{\bSigmav}{\ensuremath{\mathbf{\undertilde{\bSigma}}}}
\newcommand{\sigmav}{\ensuremath{\undertilde{\sigma}}}
\newcommand{\av}{\ensuremath{\undertilde{a}}}
\newcommand{\bav}{{\ensuremath{\mathbf{\undertilde{\ba}}}}}
\newcommand{\bcv}{{\ensuremath{\mathbf{\undertilde{\bc}}}}}
\newcommand{\bdv}{{\ensuremath{\mathbf{\undertilde{\bd}}}}}
\newcommand{\bnv}{{\ensuremath{\mathbf{\undertilde{\bn}}}}}
\newcommand{\bsv}{{\ensuremath{\mathbf{\undertilde{\bs}}}}}


\newcommand{\Uav}{\ensuremath{\undertilde{\Ua}}}
\newcommand{\bUav}{\ensuremath{\mathbf{\undertilde{\bUa}}}}
\newcommand{\bAcv}{\ensuremath{\mathbf{\undertilde{\bAc}}}}
\newcommand{\bncv}{\ensuremath{\mathbf{\undertilde{\bnc}}}}
\newcommand{\bscv}{\ensuremath{\mathbf{\undertilde{\bsc}}}}


